Communication-efficient Decentralized Machine Learning over Heterogeneous Networks

In the last few years, distributed machine learning has been usually executed over heterogeneous networks such as a local area network within a multi-tenant cluster or a wide area network connecting data centers and edge clusters. In these heterogeneous networks, the link speeds among worker nodes vary significantly, making it challenging for state-of-the-art machine learning approaches to perform efficient training. Both centralized and decentralized training approaches suffer from low-speed links. In this paper, we propose a decentralized approach, namely NetMax, that enables worker nodes to communicate via high-speed links and, thus, significantly speed up the training process. NetMax possesses the following novel features. First, it consists of a novel consensus algorithm that allows worker nodes to train model copies on their local dataset asynchronously and exchange information via peer-to-peer communication to synchronize their local copies, instead of a central master node (i.e., parameter server). Second, each worker node selects one peer randomly with a fine-tuned probability to exchange information per iteration. In particular, peers with high-speed links are selected with high probability. Third, the probabilities of selecting peers are designed to minimize the total convergence time. Moreover, we mathematically prove the convergence of NetMax. We evaluate NetMax on heterogeneous cluster networks and show that it achieves speedups of 3.7X, 3.4X, and 1.9X in comparison with the state-of-the-art decentralized training approaches Prague, Allreduce-SGD, and AD-PSGD, respectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> revision.tex <==
\onecolumn

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

%\nobalance

%\twocolumn

\begin{auxmulticols}{2}

%%% Dumi: what needs to be addressed:
%%% - Reviewer #4: Comments R1, R2, R3
%%% - Reviewer #5: Comments R1, R2, R3, R4, R5, R6
%%% - Reviewer #6: Comments R1, R2
%%%
%%% Dumi: I recommend responding to R1, R2, ... first, and then to Dx ans Wx, for each reviewer.

\noindent 

We would like to thank all the reviewers for their insightful and constructive comments. We have carefully addressed the comments and revised the paper, where major changes are highlighted in {\color{blue} blue}. Due to space constraint, we had to remove the Appendix from the main paper. In addition, we have made the \fullpaperterm{} (with the Appendix) available on \texttt{arXiv}\footnote{\label{note:full-paper}\url{\fullpaperurl}}. In what follows, we first summarize the major changes that we have made and then provide a point-by-point response to each reviewer's comments.

\subsection*{Summary of Changes}
\begin{itemize}[leftmargin=*]
    \item \textbf{Change 1.} We added an example in \autoref{sec:introduction} to enhance the motivation of the paper.
    \item \textbf{Change 2.} We added the approximation bound of \autoref{alg:get-policy} at the end of \autoref{subsection:plicy-design} and its derivation in Appendix B of the \fullpaperterm{}. This approximation bound of $\frac{U}{L}\frac{\ln(M\!-\!1)\!-\!\ln(M\!-\!3)}{\ln(1\!-\!2a\!+\!a^{M})\!-\!\ln(1\!-\!2a\!+\!a^{M\!+\!1})}$ represents the upper value of the ratio between the objective value of Eq~(\ref{eq:o0}) derived by \autoref{alg:get-policy} and the optimal value. The assumptions are that the graph connecting the worker nodes is fully-connected, the network is heterogeneous, and $a$ denotes the minimum positive entry of $\mathbb{E}[(\boldsymbol{D}^k)^{T} \boldsymbol{D}^k]$.
    \item \textbf{Change 3.} We derived the convergence rate of \ourtech{} and added the result in \autoref{theorem:converge}. Specifically, the convergence rate of \ourtech{} is $O(1/\sqrt{k})$ where $k$ is the global iteration step. The derivation can be found in Appendix E of the \fullpaperterm{}.
    \item \textbf{Change 4.} We added \autoref{subsec:netmax-extension} to discuss how to extend a Network Monitor to existing decentralized training approaches for improving the training speed.
    \item \textbf{Change 5.} We added experiments with five datasets, more models and different settings in \autoref{sec:eval}. Specifically, \autoref{subsec:probability-performance} presents experiments to explore the performance improvement brought about by the adaptive probabilities for worker nodes to choose neighbor nodes. \autoref{subsec:nonuniform-data} includes experiments of training models on five datasets with non-uniform data partitioning. \autoref{subsec:smallmodel} includes experiments of training a small model (i.e., MobileNet) on a complex dataset (i.e., CIFAR100). \autoref{subsec:extend-netmax} includes experiments of adding a Network Monitor to AD-PSGD similar to the one used in NetMax.
\end{itemize}


\subsection*{Response to Reviewer 4}

%%% Dumi: I suggest keeping only reviewer's comment under R1
%\begin{comment}
%\textbf{W1:} Authors do not show separately the impact of the parallelization of the %local computation and network communication vs. using the probabilities to choose the %faster links, on the final efficiency.
%\vspace{2mm}
%\noindent
%\textbf{D1:} It is not clear whether the achieved improvement in the efficiency is %because of the parallelization of the local computation and network communication in %each worker node or it is mostly because of the reducing the communication cost with %choosing the links with higher speed. The proportions should have been showed.
%\end{comment}

\vspace{2mm}
\noindent
\textbf{R1:} \textit{Authors should show separately the impact of the parallelization of the local computation and network communication vs. using the probabilities to choose the faster links.}

\vspace{2mm}
\noindent
\textbf{Response.} 
In \autoref{subsec:probability-performance} of the revised paper, we have added the suggested experiments to illustrate the effectiveness of the proposed two strategies in \ourtech{}. As shown in \autoref{fig:serialize-parallel}, the use of adaptive probabilities contributes to the majority of performance improvement in \ourtech{}. For ResNet18 and VGG19 models, \ourtech{} with adaptive probabilities reduces the epoch time by 44.2\% and 45.3\% respectively comparing to \ourtech{} with uniform probabilities. On the other hand, running local computation and network communication in parallel also reduces the epoch time, but the impact is minor.
This is because the time spent on the gradient computation is much smaller than the time of network communication in our setting, leading to a marginal performance gain compared with the one contributed by the adaptive probabilities.

%%% Dumi: I suggest keeping only reviewer's comment under R2
%\begin{comment}
%\vspace{2mm}
%\noindent
%\textbf{W2:} Although there is some reasons to get lower accuracy (but not higher %accuracy), \ourtech{} achieves slightly better accuracy than others. It is not clear why %that is the case.
%\vspace{2mm}
%\noindent
%\textbf{D3:} There are some reasons to get lower accuracy, but there is no reason to get %better accuracy, while the authors show that the accuracy is slightly better than others %with no clear explanation.
%\end{comment}

\vspace{2mm}
\noindent
\textbf{R2:} \textit{It should be justified why \ourtech{} has got better accuracy. Also, it should be analysed in which cases \ourtech{} can achieve better or worse accuracy.}

%%%wyc: might not be persuadable as the reviewer may argue that the imported randomness could also lead to a worse sub-optima.
%%%Dumi: The explanation is not convincing. We need to rephrase it.
\vspace{2mm}
\noindent
\textbf{Response.} 
The reason is that the adjustable probabilities for worker nodes to select neighbors introduce more randomness to the distributed training, which is more likely to drag the training out of a shallow and sharp sub-optima and then jump into a deeper and flat sub-optima~\cite{kleinberg2018an,bottou1991stochastic}. According to prior research works~\cite{neelakantan2017adding, keskar2017on}, shallow and sharp sub-optima leads to inferior generalization, and adding some randomness or noise can achieve a better sub-optima and indeed improve the performance of the trained model. For example, \cite{neelakantan2017adding} proposes to add gradient noise to improve the performance of a trained deep model. In the revised paper, we have added the above explanation in the second paragraph of \autoref{subsec:exp-convergence}.


%%% Dumi: I suggest keeping only reviewer's comment under R3. I moved R3 before D2.
%\vspace{2mm}
%\noindent
%\textbf{W3:} \ourtech{} has been tested only on a dataset which causes to have doubts about the accuracy and efficiency. Also, the proposed solution should have been checked with different configurations to see all the possible aspects.
%\vspace{2mm}
%\noindent
%\textbf{D4:} \ourtech{} has been tested only on a dataset, so does not seem to be enough. More datasets with different partitioning on the nodes are needed.

\vspace{2mm}
\noindent
\textbf{R3:} \textit{Authors should try at least five datasets to see accuracy and efficiency with different ways of partitioning the training data. The impact of the model sizes is also worthwhile to be checked. Check the \ourtech{} and other competitors on the same data and hyper parameters where the capacity of models are not enough to learn the training data (smaller number of weights and parameters), and see the difference in the accuracy and the speed of the convergence.}

\vspace{2mm}
\noindent
\textbf{Response.} 
As suggested, we have conducted additional experiments by using five datasets with different ways of data partitioning in the revised paper. These five datasets are MNIST, CIFAR10, CIFAR100, Tiny-ImageNet, and ImageNet. The experimental results in \autoref{subsec:nonuniform-data} show that \ourtech{} significantly outperforms other competitors in terms of convergence time while retaining the training accuracy.

Moreover, we also trained a small model, i.e., MobileNet, on CIFAR100. The results show that the test accuracy of MobileNet is about $63\%$, which is smaller than $71\%$ of ResNet18. The reason is that MobileNet is simpler and not able to learn as well as larger models. Even so, \ourtech{} runs much faster and achieves a similar accuracy compared to other competitors, as shown in \autoref{subsec:smallmodel}.


\vspace{2mm}
\noindent
\textbf{D2:} \textit{\ourtech{} guarantees the convergence to the same optimal point as others, but does not guarantee the better efficiency. As authors mention in the heterogeneous networks, the link speeds among workers vary significantly, and it is possible that a node becomes busy for a long time with other jobs in multi-tenant clusters, assume the way of distributing the training data is not uniform or the importance of the training data in different nodes are different. So it is likely that the most important data is located in the slowest nodes which are chosen by the neighbors with the lowest probabilities. In this case, the efficiency of converging of the \ourtech{} gets worse, and the cost of the computations may surpasses the communication cost. The proposed solution should have been examined in the case that data is not distributed uniformly among nodes, and some nodes with slowest links do not have access to some part of the data. This also may affect the accuracy as well.}

\vspace{2mm}
\noindent
\textbf{Response.} 
There are two ways for a worker node $i$ to learn from a low-link-speed neighbor $j$. First, node $i$ can either pull the model of node $j$ directly with a low selection probability or pull the models from its other neighbors (through which the model information of node $j$ can be propagated to node $i$). 
Second, in \ourtech{}, a worker node would assign a higher weight to the pulled models from neighbors with lower selection probabilities. As described in lines~\ref{code:l11}-\ref{code:l13} of \autoref{alg:nadsgd},
the model update rule can be rewritten as
\[
x_i^{k+1}=\Big(1-\alpha\rho\frac{d_{i,m}+d_{m,i}}{2p_{i,m}}\Big)(x_{i}^{k}-\alpha g_{i}^{k})+ \alpha\rho \frac{d_{i,m}+d_{m,i}}{2p_{i,m}}x_{m}^{k}
\]
From the second item of the right-hand side, if node $i$ chooses neighbor node $m$ with a small probability $p_{i,m}$, then the update rule will assign a higher weight to the pulled model $x_m^k$ from neighbor $m$ and the updated model can maintain more information from neighbor $m$. Therefore, even if node $i$ pulls the model from $m$ with a low probability, such an update rule can help $i$ maintain enough information from $m$.

As advised, we have conducted more experiments to evaluate the non-uniformly partitioned training data on five datasets. The experimental results are presented in \autoref{subsec:nonuniform-data}. 
We observe that the distribution of training data affects the training accuracy and convergence efficiency of all the approaches including \ourtech{}.
On the other hand, \ourtech{} achieves comparable accuracy and convergence efficiency in terms of iterations, and outperforms the competitors significantly in terms of convergence time. 
The performance gain of \ourtech{} mainly comes from the two factors described above. 

%First, a node $i$ can obtain the model information of a low-speed-link neighbor node $j$ from other neighbors. This is because the other neighbors can pull the model from $j$ and update their local model by using $j$'s model. As a result, the models of the other neighbors contain the model information of $j$, and when node $i$ pulls the models of the other neighbors, the model information of $j$ can be propagated to node $i$. 
%In general, the above two factors can help any node to obtain sufficient information from other nodes, leading to high efficiency and accuracy of the training even with skewed data partitioning. 


\vspace{10pt}
\subsection*{Response to Reviewer 5}
\vspace{2mm}
\noindent
\textbf{R1:} \textit{Please explain why prior approaches that use static communication probabilities cannot be simply extented with a Network Monitor to adapt communication similarly to \ourtech{}. If they can, please provide experimental results on their performance. If not, please explain why.}

\vspace{2mm}
\noindent
\textbf{Response.}
In the revised paper, we show that if an approach can be formulated in the form of Eq.~(\ref{eq:j1}), then it can be extended with a Network Monitor similar to \ourtech{}. 
The extension includes two steps. 
%First, by letting the entry $y_{i,m}$ of $\mathbb{E}[(\boldsymbol{D}^k)^{T} \boldsymbol{D}^k]$ to be larger than 0, for all $d_{i,m}\neq 0$, we can derive a new constraint Eq. (\ref{eq:o3}). Second, resolving the optimal problem stated in Eq. (\ref{eq:o0})-(\ref{eq:o5}), we obtain the probabilities for worker nodes to choose neighbors. 
First, we can derive a similar constraint to replace Eq.~(\ref{eq:o3}) by requiring each entry $y_{i,m}$ of $\mathbb{E}[(\boldsymbol{D}^k)^{T} \boldsymbol{D}^k]$ to be larger than $0$, for all $d_{i,m}\neq 0$. 
Second, the corresponding probabilities for worker nodes to choose neighbors can be obtained by solving the optimization problem stated in Eq.~(\ref{eq:o0})-(\ref{eq:o5}). 
By doing so, the approaches can be enhanced to adapt to dynamic heterogeneous networks. 
\par
In the revised paper, we added \autoref{subsec:netmax-extension} to discuss such extension, as well as new experiments based on AD-PSGD to demonstrate its effectiveness in \autoref{subsec:extend-netmax}.

%%% === R2 ===
%\vspace{2mm}
%\noindent
%\textbf{D2:} Could you include in a graph the performance of a parameter server implementation, as a baseline which is considered straightforwardly worse in terms of training time? see also D6.

\vspace{2mm}
\noindent
\textbf{R2:} \textit{In the experimental evaluation, include in one or more graphs the performance of a parameter server implementation, as a baseline.}

\vspace{2mm}
\noindent
\textbf{Response.}
In the revised paper, we have added an implementation of a parameter server (PS) as another baseline in \autoref{subsec:smallmodel}. The results show that PS with synchronous/asynchronous training performs worse than the other approaches. This is mainly due to the high communication cost between the PS and the worker nodes.

%%% === R3 ===
%\vspace{2mm}
%\noindent
%\textbf{D3:} In figure 8, it seems that increasing the number of nodes also increases the resulted speedups of \ourtech{}. Therefore, I would like to see some results with more than 16 nodes. If the same trend continuous then this will strengthen the contribution of the paper and will exhibit enhanced scalability compared to other approaches.

\vspace{2mm}
\noindent
\textbf{R3:} \textit{In figure 8, provide results with more than 16 nodes.}

\vspace{2mm}
\noindent
\textbf{Response.} 
We have added new experiments with $20$ worker nodes, as shown in \autoref{fig:speedup} of the revised paper. The results show that the speedup of \ourtech{} is consistent with that of using less than $16$ worker nodes.

%%% === R4 ===
%\vspace{2mm}
%\noindent
%\textbf{D5:} Could you explain why you do not use any common benchmark suite for learning in decentralized settings, in your experimentation?

\vspace{2mm}
\noindent
\textbf{R4:} \textit{Explain why you do not use any common benchmark suite for learning in decentralized settings in your experimentation}

\vspace{2mm}
\noindent
\textbf{Response.}
In the earlier submitted version, we used the models and datasets adopted by the papers of the competitors. In the revised version, we have additionally used the benchmark suite for image classification proposed by MLPerf~\cite{Mattson2020}. Specifically, we added new experiments of training the ResNet50 model on the ImageNet dataset. The experimental results are presented in \autoref{subsec:nonuniform-data}. 

%%% === R5 ===
%\vspace{2mm}
%\noindent
%\textbf{D6:} Have your measured how far is the "feasible communication policy" from the optimal ones even in simplified setups? is there any guarantee or empirical conclusion on how far feasible is from optimal?

\vspace{2mm}
\noindent
\textbf{R5:} \textit{Have your measured how far is the "feasible communication policy" from the optimal ones in a simplified setup or state it theoretically the approximation factor, if possible.}

\vspace{2mm}
\noindent
\textbf{Response.} 
When the network is homogeneous, the worker nodes of \ourtech{} will choose each neighbor with uniform probabilities. According to Boyd's research~\cite{boyd2006randomized}, \ourtech{} can achieve the optimal convergence rate as well as the optimal objective value of Eq~(\ref{eq:o0}).

When the network is heterogeneous, if the graph connecting the worker nodes is fully-connected, the approximation factor is $\frac{U}{L}\frac{\ln(M\!-\!1)\!-\!\ln(M\!-\!3)}{\ln(1\!-\!2a\!+\!a^{M})\!-\!\ln(1\!-\!2a\!+\!a^{M\!+\!1})}$, where $a$ is the minimum positive entry of $\mathbb{E}[(\boldsymbol{D}^k)^{T} \boldsymbol{D}^k]$. The approximation factor is correlated to the network condition as well as the number of worker nodes $M$. 
\ifthenelse{\boolean{isfullpaper}}
{
The detailed proof is presented in Appendix \ref{apendex:a-1}.
}
{
The detailed proof is presented in Appendix B of the \fullpaperterm{}.
}


%%% === R6 ===
%\vspace{2mm}
%\noindent
%\textbf{D7.} The parameter server model provides a number of desirable features and value added services, such as Interaction with user via the server at the very same time the training goes on, simultaneous application of currently extracted models to unlabeled data, monitoring state, on-the-fly reconfiguration and provisioning of resources (e.g. addition of worker nodes or freeing some of them), use of synchronous, asynchronous and dynamic averaging synchronization policies etc. Could you state which of these properties are preserved here and which cannot?

\vspace{2mm}
\noindent
\textbf{R6.} \textit{Clearly explain which facilities provided by the parameter server, as noted in D7, are maintained in your scheme. For instance, I want to label unlabeled data based on the currently maintained model. Could i do that? which node in the distributed setting do i have to query?}

\vspace{2mm}
\noindent
\textbf{Response.}
The functionalities provided by the parameter server can also be implemented in \ourtech{}. For example, we can implement these functionalities in the Network Monitor of \ourtech{}.
%%% ooibc: properties?
%%% --> functionalities
%--> have replaced "properties" with "functionalities"
By doing so, the Network Monitor can interact with users, retrieve models from the worker nodes (e.g., choose the best one or the average of all models), monitor training state, reconfigure and provision resources on-the-fly, choose synchronous or asynchronous decentralized training algorithms, as well as dynamic averaging synchronization. 

If a user wants to label unlabeled data based on the currently maintained model, she or he can send request to the Network Monitor to retrieve a model from the worker nodes, e.g., using one of the following three ways: (1) choose a model from any worker node, (2) choose the best model from the worker nodes, or (3) choose the average model of all worker nodes.

%%% === R7 ===
%\vspace{2mm}
%\noindent
%\textbf{D4:} If possible, I would have liked to see results within an actual multi-site cloud setting, e.g. via AWS or Azure.

\vspace{2mm}
\noindent
\textbf{R7:} \textit{(optional) I would have liked to see results within an actual multi-site cloud setting, e.g. via AWS or Azure.}

\vspace{2mm}
\noindent
\textbf{Response.}
In the revised paper, we have added a set of experiments across $6$ Amazon EC2 regions. In each region, we used a \textit{c5.4$\times$large} instance as a worker node. 
We trained two CNN models (i.e., MobileNet and GoogLeNet) on the MNIST dataset to evaluate the performance of \ourtech{}.
%The worker nodes collaboratively train a model by communicating through the Wide Area Network connecting the EC2 regions. 
The results show that \ourtech{} converges approximately $2\times$ faster than the other competitors. 
Due to the space constraint, we present these experimental results in Appendix G of the \fullpaperterm{}.



%%% === W1 ===
\vspace{2mm}
\noindent
\textbf{W1:} \textit{the experimental results frequently do not show so great an improvement over the second best competitor. The training speedup, communication cost etc is indeed UP TO x3.7 but this is not the average case.}

\vspace{2mm}
\noindent
\textbf{Response.}
The performance of \ourtech{} is close to the performance of the second-best competitor (AD-PSGD) over homogeneous networks since they have similar communication models. However, \ourtech{} outperforms AD-PSGD by $2\times$ when the network is heterogeneous. Such an improvement is due to the optimized utilization of high-speed links. For the training speedup, \ourtech{} outperforms the other competitors by $3\times$ on average.

%%%Will: {\color{red}(Is it OK to response like this?) }

%%% === W2 ===
%%% Dumi: I think there is no need to respond to W2 since it is half-appreciative.
%\vspace{2mm}
%\noindent
%\textbf{W2:} The discussed ideas such as the consensus SGD algorithm and the communication policy are not that novel and exciting. We have simple concepts here (at the core of \ourtech{}, just adjustable communication probabilities) that are nicely put together.

%\vspace{2mm}
%\noindent
%\textbf{Response.}
%First, unlike previous decentralized approaches that simply average local model and pulled model every iteration, the update rule of consensus SGD gives higher weight to pulled models from neighbors chosen with lower probabilities, which can enhance the model information from low-link-speed neighbors even the local node has a long time not to pull the model from low-link-speed neighbors. Such a design can improve the convergence rate intuitively, as the experiment shown in \autoref{subsec:extend-netmax}. Second, unlike most of previous training approaches that are aimed to maximum the convergence rate while ignoring the duration time per iteration, the probabilities of \ourtech{} seek a trade-off between convergence rate and duration time per iteration to minimize the convergence time). Third, adaptively tuning the probabilities requires measuring the changes of link-speeds in real-time. Traditional way to measure the link-speeds require injecting large amount of traffic into the network to detect the link speeds. This can waste transmission capacities of the communication links and significantly impacts the data transfers of the distributed training. In contrast, \ourtech{} utilizes the communication of distributed training to detect the changes of link speeds, which avoids wasting the transmission capacities of communication links.



\vspace{10pt}
\subsection*{Response to Reviewer 6}
\vspace{2mm}
%%% === W1/R1 ===
\noindent
\textbf{W1.} \textit{The motivation of this paper needs to be improved. I think it is better to give a concrete example in the introduction.}

\vspace{2mm}
\noindent
\textbf{R1.} \textit{Fix W1}

\vspace{2mm}
\noindent
\textbf{Response.}
%We have added an example to illustrate the limitations of advanced decentralized learning approaches. Please see the Paragraph 1 at the left column on Page 2.
We have added an example in \autoref{fig:example-bottleneck-2} of the revised paper to illustrate the limitations of existing asynchronous D-PSGD approaches and refined the presentation in \autoref{sec:introduction} to improve the motivation.
Essentially, in a dynamic heterogeneous network, existing centralized and decentralized training approaches suffer from the low-speed links. 
Therefore, our motivation is to design an adaptive training approach that can fully utilize the high-speed links to improve the communication efficiency.

%%% === R2/W3 ===
\vspace{2mm}
\noindent
\textbf{W3.} \textit{In the experiment section, it seems that the authors only do experiments on CIFAR10 dataset but not on ImageNet dataset. However, in the papers of AllReduce [2], Prague [3] and AD-PSGD [1], they all have experiments on ImageNet. Thus, we require the author to do the experiments on ImageNet dataset.}

\vspace{2mm}
\noindent
\textbf{R2.} \textit{Fix W3}

\vspace{2mm}
\noindent
\textbf{Response.} 
We have added new experiments on the ImageNet dataset, as shown in \autoref{subsec:nonuniform-data} of the revised paper. The experimental results are consistent with those of the experiments on CIFAR10 dataset. 
%Please see \autoref{subsec:nonuniform-data}.


%%% === R3/W2 ===
\vspace{2mm}
\noindent
\textbf{W2.} \textit{In the section of convergence analysis, It is better to give the convergence rate with respect to the number of iterations like AD-PSGD [1].}

\vspace{2mm}
\noindent
\textbf{R3.} \textit{Fix W2 (optional; but at least try)}

\vspace{2mm}
\noindent
\textbf{Response.}
If the learning rate is given as a constant $c/\sqrt{k}$ where $c$ is a positive constant and $k$ represents the global iteration steps, the convergence rate of \ourtech{} is $O(1/\sqrt{k})$ which is similar to AD-PSGD. We have added the result in \autoref{theorem:converge} and provided the detailed proof in Appendix E of the \fullpaperterm{}.


\end{auxmulticols}

\twocolumn

==> sec-evaluation.tex <==
\section{Performance evaluation}
\label{sec:eval}

% In this section, we evaluate the performance of our approach. 
% We describe the experimental setup in \autoref{subsec:exp-setup}, and present the evaluation results for both heterogeneous and homogeneous networks in \autoref{subsec:exp-hetero} and \autoref{subsec:exp-homo}, respectively.

\subsection{Experimental Setup}\label{subsec:exp-setup}

\noindent\textbf{Environment.} 
Experiments are conducted in a multi-tenant cluster consisting of $18$ servers, which are connected by $1000$ Mbps Ethernet. 
%%% linqian0617: how many master and worker nodes are there respectively? 
%%% Pan: there is only a master node, the numbers of worker nodes are 4,8,16, respectively, described in the following sub-section.
Each server is equipped with $3$ or $8$ GPUs, as shown in \autoref{tab:serverconfig}. 
We run the worker nodes in docker containers, and each node uses one GPU. 
%
To emulate a heterogeneous network, some links are slowed down, as described in \autoref{subsec:exp-hetero}.

\begin{table}[tp]
	\centering
	\caption{Configuration of each GPU server}
	\begin{tabular}{l|l}
		\hline
		Processor& 1$\times$ Intel(R) Xeon(R) W-2133 CPU @ 3.60GHz\\
		\hline
		Memory size& 65GB \\
		\hline
		GPUs&3$\times$ or 8$\times$ GeForce RTX 2080 Ti\\
		\hline
		Network&1000 Mbps Ethernet\\
		\hline
		Operating system&Ubuntu 16.04 LTS\\
		\hline
	\end{tabular}
	\label{tab:serverconfig}
	\vspace{-2ex}
\end{table}

\noindent\textbf{Models and dataset.} 
We train two CNN models, namely ResNet18 and VGG19, on the CIFAR10 dataset, to evaluate the performance of our proposed approach. 
The model sizes of ResNet18 and VGG19 are approximately 50MB and 500MB, respectively. 
The CIFAR10 dataset consists of $50,000$ training images and $10,000$ testing images with size of $32 \times 32$ pixels. 
% Though CIFAR10 only has 10 classes, the images are complex enough. Importantly, we can compare the converged performance of the models within acceptable experiment time.

\noindent\textbf{Baselines.}
We compare \ourtech{} with three state-of-the-art decentralized approaches, including Allreduce-SGD~\cite{jia2018highly}, 
%the heterogeneity-tolerant algorithms 
AD-PSGD~\cite{lian2018asynchronous} and Prague~\cite{luo2020prague}. 
For a fair comparison, we implement the four approaches in PyTorch such that they share a similar runtime environment. 
For all the approaches, we use the widely adopted hyper-parameter settings as applied in AD-PSGD~\cite{lian2018asynchronous} and Prague~\cite{luo2020prague}. 
Specifically, we train the models with \emph{batch size} $128$, \emph{momentum} $0.9$, and \emph{weight decay} $10^{-4}$. 
The \emph{learning rate} starts from $0.1$ and decays by a factor of $10$ once the loss does not decrease any more. 
We train ResNet18 and VGG19 with \emph{epoch numbers} of $64$ and $82$ respectively. 
For \ourtech{}, we update the communication policy every $T_s = 2$ minutes since this period is long enough to detect the change of link speed.

\subsection{Performance in Heterogeneous Network}\label{subsec:exp-hetero}

\noindent\textbf{Network settings.} 
We randomly slow down one of the communication links among nodes by 2$\times$-10$\times$, similar to AD-PSGD~\cite{lian2018asynchronous}. 
Other than that, we further change the slow link every $5$ minutes. 
As the processing time of distributed machine learning jobs varies from tens of minutes to several days~\cite{lian2018asynchronous, jeon2019analysis}, the above frequency of link speed change is appropriate to mimic the dynamic arriving/leaving of learning jobs in a multi-tenant cluster. 
Due to the limited number of GPUs available on each server, we run $4$, $8$ and $16$ worker nodes across $2$, $3$ and $4$ servers, respectively. 
Unless otherwise specified, the number of worker nodes is $8$ by default. 

\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:epoch-time:a}     \includegraphics[width=1\textwidth]{epoch-time-resnet-hetero} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:epoch-time:b}     \includegraphics[width=1\textwidth]{epoch-time-vgg-hetero} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Average epoch time with 8 worker nodes in a heterogeneous network.}
	\label{fig:epoch-time}
	\vspace{-1ex}
\end{figure}

\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:loss-time:a}     \includegraphics[width=1\textwidth]{resnet-loss-time} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:loss-time:b}     \includegraphics[width=1\textwidth]{vgg-loss-time} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Training loss with 8 worker nodes in a heterogeneous network.
	}
	\label{fig:loss-time}
	\vspace{-1ex}
\end{figure}



%%% Dumi: I suggest removing this to save space and add the communication/computation time.
%%% Pan: In the figure presenting epoch time, I break the epoch time into communication/computation time
\begin{comment}
\noindent\textbf{Convergence \textit{w.r.t.} epochs.}
Fig.~\ref{fig:loss-epoch} shows the comparison of training loss \textit{w.r.t.} epochs. 
We can observe that the losses of Allreduce-SGD and Prague decrease slightly faster than those of AD-PSGD and \ourtech{}, which means the former two algorithms converge more quickly in terms of epoch. 
However, as we discussed in \autoref{subsection:plicy-design}, a faster epoch convergence rate does not necessarily lead to shorter training time because the time of each epoch is also a determining factor, which we will demonstrate it in \autoref{fig:loss-time}. 
In addition, the ResNet18 model converges much faster than VGG19 in all the algorithms because ResNet18 adopts the residual network to accelerate the convergence.
\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:loss-epoch:a}     \includegraphics[width=1\textwidth]{resnet-loss-epoch} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:loss-epoch:b}     \includegraphics[width=1\textwidth]{vgg-loss-epoch} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Training loss with 8 worker nodes in a heterogeneous network.%%%wyc: (removal) Losses of Allreduce and Prague decrease fastest with epochs. Losses of AD-PSGD and \ourtech{} decreases slightly slower than that of Allreduce and Prague.
	}
	\label{fig:loss-epoch}
	%\vspace{-1ex}
\end{figure}
\end{comment}


%%%Will: I replace the original figures of epoch time by new ones which break the epoch time into communication and computation
\noindent\textbf{Computation cost \textit{vs.} communication cost.}
\autoref{fig:epoch-time} presents the computation cost and communication cost of average epoch time of the four approaches. 
The computation costs of the four approaches are almost the same since they train the same model under the same runtime environment. 
However, communication costs differ significantly. 
In particular, \ourtech{} has the lowest communication cost since it can fully utilize the high-speed links. 
For ResNet18, \ourtech{} reduces the communication cost by up to $83.4\%$, $81.7\%$, and $63.7\%$ comparing with Prague, Allreduce-SGD, and AD-PSGD, respectively. 
For VGG19, \ourtech{} reduces the communication cost by up to $76.8\%$, $69.2\%$, and $58.6\%$, correspondingly.  
%
Prague suffers from the highest communication cost. 
This is because Prague divides the worker nodes into multiple groups in every iteration, and each group executes a \textit{partial-allreduce} operation to average the models.
The concurrent executions of partial-allreduce of different groups compete for the limited bandwidth capacity, resulting in network congestion. 
%Besides, the partial-allreduce operation of each group still suffers from low-speed links. 
Moreover, the partial-allreduce operation is agnostic to the link speed. As a consequence, the heavy use of low-speed links further deteriorates the performance.
%As a result, the communication cost of Prague is high. 

\noindent\textbf{Convergence \textit{w.r.t.} time.} 
\autoref{fig:loss-time} shows the comparison of training loss \textit{w.r.t.} time. 
\ourtech{} converges much faster than the other approaches in terms of training time. For ResNet18, \ourtech{} achieves about 3.7$\times$, 3.4$\times$, and 1.9$\times$ speedup over Prague, Allreduce-SGD, and AD-PSGD, respectively. For VGG19, the speedup is about 2.8$\times$, 2.2$\times$, and 1.7$\times$ over the other three approaches, respectively. The reason is that \ourtech{} enables the worker nodes to communicate preferably with neighbors over high-speed links, and, thus, reduces the communication cost. As a consequence, \ourtech{} can iterate much faster than the other approaches.

\noindent\textbf{Speedup \textit{w.r.t.} number of worker nodes.} \ourtech{} has better scalability than the other three approaches over heterogeneous networks. 
%%%wyc: please check here, Fig. 6 seems to be the comparison to all approaches by varying the number of worker nodes
For better illustration, we use the training time after finishing a given epoch in Allreduce-SGD with 4 worker nodes as a baseline and show the speedup of all approaches over this baseline with varying number of nodes in \autoref{fig:speedup}. The given epoch is set to 64 and 82 for ResNet18 and VGG19, respectively.
%
We observe that \ourtech{} always has the best speedup, and the advantage enlarges as the number of worker nodes increases. 
%
%For instance, for 4 worker nodes, the speedup of \ourtech{}, Prague, AD-PSGD, and Allreduce-SGD are xx, xx, xx, and xx, respectively. While for 16 worker nodes, the speedup of the four approaches are xx, xx, xx, and xx, respectively. 
%
The other three approaches perform worse than \ourtech{} in terms of speedup because they experience a higher communication cost in a heterogeneous network. 

%%%wyc: if all algorithms have the same effect, the comparison might not be interesting, we may need to present the superiority of \ourtech{}
%%% Pan: As \ourtech{} takes much less time to converge, reviews may curious about the final accuracy of the trained model. If the accuracy is too low, then \ourtech{} is not a good approach. Therefore, the accuracy here shows that \ourtech{} can train much faster without loss any accuracy, which also means \ourtech{} can achieve the same accuracy with much less time.
%%%wyc: I mean, the accuracy of \ourtech{} is also higher, we may emphasize that.
\noindent\textbf{Accuracy.} 
\autoref{tab:acc-hetero} summarizes the test accuracy of all the approaches after finishing the given epochs. 
%
All the approaches achieve around 90\% test accuracy for both ResNet18 and VGG19, while \ourtech{} performs slightly better than the other approaches. 
%
%In fact, the accuracy of \ourtech{} is slightly higher than that of the other approaches. Table \ref{tab:acc-hetero} shows that all the approaches achieve test accuracy of about 90\% after finishing the given epochs, for both ResNet18 and VGG19.

\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:speedup:a}     \includegraphics[width=1\textwidth]{resnet-speedup} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:speedup:b}     \includegraphics[width=1\textwidth]{vgg-speedup} } 
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Speedup \textit{w.r.t.} number of worker nodes in a heterogeneous network.}
	%%%wyc: is this figure caption wrong? (I edited here, previous caption: Speedup compared to Allreduce with 4 worker nodes in a heterogeneous network.)
	% The speedup on execution time of finishing given epochs compared to Allreduce with 4 worker nodes. For all algorithms, we train ResNet18 and VGG19 with epoch number 64 and 82, respectively. Different number of worker nodes over heterogeneous network.}
	\label{fig:speedup}
	\vspace{-1ex}
\end{figure}

\begin{table}[tp] \scriptsize
	\newcommand{\multirow}
	\centering
	\caption{Accuracy of models trained over a heterogeneous network}
	\begin{tabular}{ll|l|l|l|l}
		\hline
		&&Prague&Allreduce&AD-PSGD&\ourtech{}\\
		\hline
		                         &4 nodes&89.56\%&90.11\%&90.24\%&90.46\%\\	
	                     ResNet18&8 nodes&90.54\%&90.16\%&90.39\%&91.14\%\\
		                         &16 nodes&90.44\%&90.37\%&90.23\%&90.78\%\\
		\hline
		                         &4 nodes&90.09\%&89.98\%&89.8\%&90.24\%\\	
		                 VGG19&8 nodes&89.76\%&89.05\%&90.47\%&90.74\%\\
		                         &16 nodes&90.14\%&90.13\%&90.22\%&91.07\%\\
		\hline
	\end{tabular}
	\label{tab:acc-hetero}
	\vspace{-1ex}
\end{table}

\subsection{Performance in Homogeneous Network}\label{subsec:exp-homo}
\noindent\textbf{Network settings.} To emulate a homogeneous network and avoid network competition with other jobs in the cluster, we reserve a server with 8 GPUs and run 4, 6, and 8 worker nodes within the server, respectively. The worker nodes are connected by a virtual switch \cite{ovs} with 10Gbps bandwidth to communicate with each other in a homogeneous way.

%%% Dumi: Again, I suggest removing this sub-section. I commented it out
\begin{comment}
\noindent\textbf{Convergence \textit{w.r.t.} epochs.} All the algorithms have a similar convergence rate. Allreduce-SGD converges slightly faster than the other algorithms, as shown in Fig. \ref{fig:loss-epoch-homo}. For all algorithms, RenNet18 converges faster than VGG19.
\begin{figure}[bp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:loss-epoch-homo:a}     \includegraphics[width=1\textwidth]{loss-epoch-resnet-homo} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:loss-epoch-homo:b}     \includegraphics[width=1\textwidth]{loss-epoch-vgg-homo} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Training loss with 8 worker nodes in a homogeneous network.}
	\label{fig:loss-epoch-homo}
	%\vspace{-1ex}
\end{figure}
\end{comment}

%%%Pan: I add new figures which present communication and computation cost
\noindent\textbf{Computation cost \textit{vs.} communication cost.}
\autoref{fig:epoch-time-homo} presents both the computation and communication cost of the average epoch time of the four approaches. The computation costs of the four approaches are almost the same. The communication costs are significantly lower compared to those in \autoref{fig:epoch-time} due to the larger bandwidth of the network. In general, \ourtech{} and AD-PSGD have much smaller communication costs than Prague and Allreduce-SGD. 
%
This is because of that Allreduce-SGD and Prague average gradients or model parameters from multiple worker nodes in each iteration. This requires multiple rounds of communication between worker nodes, resulting in high communication costs. 
%
In contrast, each worker node in \ourtech{} and AD-PSGD pulls the model from only one neighbor and starts its next iteration once that communication is finished, which leads to low communication costs.
%Because Allreduce-SGD averages the gradients of all worker nodes every iteration and Prague averages models of partial worker nodes every iteration. Each worker node of Prague and Allreduce-SGD has to wait for the communication between other nodes to finish the gradients averaging. 
%
%In contrast, each worker node of \ourtech{} and AD-PSGD communicate with only one neighbor and starts its next iteration once the communication is finished, which has much smaller communication cost than averaging gradients of multiple nodes.
%
%In Fig. \ref{fig:epoch-time-homo}, we also observe that Prague is faster than Allreduce. This is because each worker node of Prague only waits for communication of partial worker nodes. Moreover, as the network bandwidth is large enough, the data flows of multiple allreduce operations hardly cause network congestion. As a result, Prague experience smaller communication cost than Allreduce.

\noindent\textbf{Convergence \textit{w.r.t.} time.}
\autoref{fig:loss-time-homo} shows that \ourtech{} has the fastest convergence time compared to the other approaches. For ResNet18, \ourtech{} is about 3.2$\times$, 3.5$\times$, and 1.2$\times$ faster than Prague, Allreduce-SGD, and AD-PSGD, respectively. For VGG19, \ourtech{} is about 2.0$\times$, 1.5$\times$, and 1.1$\times$ faster than Prague, Allreduce-SGD, and AD-PSGD, respectively. Note that the convergence trend of \ourtech{} and AD-PSGD are similar as these two approaches have a similar communication mode.
%%%wyc: might be better to add specific mode to explain their superiority
%%%Pan: explanation added in the communication/computation cost part
In contrast, Allreduce-SGD and Prague converge much slower since they have much higher communication costs than \ourtech{} and AD-PSGD. 
%%%wyc: why Prague that averages partial gradients still has a high cost?
%%%Pan: this explanation is added in the following comparison between communication cost and computation cost

\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:epoch-time-homo:a}     \includegraphics[width=1\textwidth]{epoch-time-resnet-homo} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:epoch-time-homo:b}     \includegraphics[width=1\textwidth]{epoch-time-vgg-homo} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Average epoch time with 8 worker nodes in a homogeneous network.}
	\label{fig:epoch-time-homo}
	\vspace{-1ex}
\end{figure}


\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:loss-time-homo:a}     \includegraphics[width=1\textwidth]{loss-time-resnet-homo} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:loss-time-homo:b}     \includegraphics[width=1\textwidth]{loss-time-vgg-homo} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{Training loss with 8 worker nodes in a homogeneous network.}
	\label{fig:loss-time-homo}
	\vspace{-1ex}
\end{figure}

\noindent\textbf{Speedup \textit{w.r.t.} number of worker nodes.} \ourtech{} has better scalability than the other three approaches in a homogeneous network. 
%%%wyc: same as Fig. 6, why here is the comparison to Allreduce with 4 nodes?
%%%Pan: this is equal to normalize the speedup to Allreduce with 4 nodes. On one hand, for the same approach, we can compare the speedups of using different number of worker nodes. On the other hand, we can easily compare the speedup of different approaches using the same worker nodes.
Similar to \autoref{fig:speedup}, we use the Allreduce-SGD with 4 worker nodes as a baseline and report the speedup over this baseline.
%Fig. \ref{fig:speedup-homo} shows the speedup compared to the baseline (i.e., Allreduce-SGD with 4 nodes) after finishing the given epochs. 
\ourtech{} and AD-PSGD have similar speedups since their communication modes are similar. 
In contrast, Allreduce-SGD and Prague perform worse than \ourtech{} and AD-PSGD in terms of speedup because of higher communication costs.


%%%wyc: maybe we could emphasize that our approach could achieve better accuracy after a given number of epoch, since I find the accuracy of \ourtech{} is higher than the others in most cases
\noindent\textbf{Accuracy.}
%\ourtech{} achieves better speedup without losing accuracy. 
As shown in Table \ref{tab:acc-homo}, for both ResNet18 and VGG19, all the approaches achieve test accuracy of around 90\% after finishing the given epochs. 
However, \ourtech{} achieves slightly higher accuracy than the other approaches in most cases.
%%% linqian0617: what's the accurcy when the datasets are applied with traditional centralized training?


\begin{figure}[tp]
	\centering 
	\begin{minipage}[b]{0.23\textwidth}
		\centering
		\subfigure[ResNet18] { \label{fig:speedup-homo:a}     \includegraphics[width=1\textwidth]{resnet-speedup-homo} }
		\vspace{-2ex}
	\end{minipage}
	\hspace{0.01in}
	\begin{minipage}[b]{0.23\textwidth}
		\centering 
		\subfigure[VGG19] { \label{fig:speedup-homo:b}     \includegraphics[width=1\textwidth]{vgg-speedup-homo} }  
		\vspace{-2ex} 
	\end{minipage} 
	\caption{
	%%% Dumi: keep it short. The details are in the text.
	Speedup \textit{w.r.t.} number of worker nodes in a homogeneous network.}
	%The speedup on execution time of finishing given epochs compared to Allreduce with 4 worker nodes. For all algorithms, we train ResNet18 and VGG19 with epoch number 64 and 82, respectively. Different number of worker nodes over homogeneous network.}
	\label{fig:speedup-homo}
	\vspace{-1ex}
\end{figure}

\begin{table}[tp]\scriptsize
	\newcommand{\multirow}
	\centering
	\caption{Accuracy of models trained over a homogeneous network}
	\begin{tabular}{ll|l|l|l|l}
		\hline
		&&Prague&Allreduce&AD-PSGD&\ourtech{}\\
		\hline
		&4 nodes&89.37\%&89.45\%&89.83\%&90.19\%\\	
		ResNet18&6 nodes&89.65\%&90.25\%&90.17\%&89.98\%\\
		&8 nodes&90.32\%&90.16\%&89.95\%&90.24\%\\
		\hline
		&4 nodes&89.97\%&90.41\%&90.69\%&90.62\%\\	
		VGG19&6 nodes&91.02\%&90.52\%&90.88\%&91.07\%\\
		&8 nodes&89.62\%&89.86\%&90.30\%&90.47\%\\
		\hline
	\end{tabular}
	\label{tab:acc-homo}
	\vspace{-2ex}
\end{table}


==> sec-introduction.tex <==
\section{Introduction}
%Recently machine learning (ML) has successfully applied in many domains to extract information from big data. It is common to train a model on large-scale dataset in distributed manner where the dataset is split into multiple partitions and feed into different worker nodes to perform parallel training. Each worker occupies a local copy of the model and trains the model copy on the allocated data partition. To ensure the correctness of the training, the workers have to communicate with each other every iteration to synchronize their models.

In real-world applications, distributed machine learning is usually executed over heterogeneous networks, such as a local area network (LAN) within multi-tenant clusters~\cite{xiao2018gandiva, jeon2019analysis} and a wide area network (WAN) across data centers or edge clusters~\cite{hsieh2017gaia}.
%
In these heterogeneous networks, the link speeds among worker nodes are highly different.
%
For machine learning model training in a multi-tenant cluster, one of the main challenges is avoiding resource fragmentation by allocating adequate co-located GPUs for worker nodes~\cite{jeon2019analysis}.
%
Often, the allocated GPUs are placed across machines or even racks~\cite{gu2019tiresias}. 
%
The link speeds within a machine differ from those across machines or racks significantly due to different capacities of the underlying infrastructure. 
%
Moreover, the network contention among distributed learning jobs can easily cause network congestion even on a 100 Gbps network, making the difference in link speeds more significant~\cite{gu2019tiresias, xiao2018gandiva}. 
%
For model training across data centers or edges, the link speeds of WAN connecting the workers are mainly determined by the geographic distance. 
%
For example, the link speed between geographically-close data centers or edges could be up to 12$\times$ faster than that between distant ones~\cite{zhou2019privacy}.

%In reality, many organizations are interested in training a high quality machine learning model over a large-scale globalized data collected from multiple sources. For example, recommender systems rely on the maximum breadth of data to overcome the cold start problems \cite{cano2016towards}, banks from different regions collaboratively train anomaly detection models for fraud detection \cite{kairouz2019advances}, and hospitals collaboratively train better diagnostic models \cite{boughorbel2019federated}. A traditional method to train such a model is to gather all the data into a data center and perform distributed training within that data center by the high-speed local area network (LAN). However, due to data protection regulations and privacy concerns \cite{kairouz2019advances}, these data cannot be shared among countries or organizations. Therefore, distributed training across multiple organizations or data centers in different countries without exchanging the raw data is essential. Unfortunately, for the differences in physical topology and network traffic, the bandwidth of wide area network (WAN) connecting the distributed data centers is highly heterogeneous and is up to 60$\times$ slower than the bandwidth of LAN within data centers \cite{hsieh2017gaia}\cite{zhou2019privacy}. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.46\textwidth]{example-bottleneck}
	\caption{Communication topology of C-PSGD and D-PSGD. For C-PSGD, worker nodes communicate with centralized parameter server to synchronize their training. For D-PSGD, worker nodes communicate with each other in a graph. Both C-PSGD and D-PSGD might be limited by low-speed links.}
	\label{fig:example-bottleneck} %% label for entire figure
	\vspace{-2ex}
\end{figure}

A highly heterogeneous network hinders machine learning approaches from efficient model training.
%
Both centralized and decentralized training approaches might be limited by low-speed links.
%
On the one hand, centralized parallel stochastic gradient descent (C-PSGD), widely implemented by various frameworks, such as TensorFlow \cite{agarwal2019static} and Apache SINGA~\cite{ooi2015singa}), requires a centralized node called parameter server to maintain a global model.
%
At each iteration, all the worker nodes exchange information (i.e., parameters and gradients) with the parameter server to update the global model, as shown in \autoref{fig:example-bottleneck}(a).
%
The worker nodes cannot start the next iteration until the information exchanges are finished. 
%
Therefore, the training progress of C-PSGD is constrained by both (1) the network congestion at the centralized node and (2) worker nodes with low link speeds.
%
On the other hand, state-of-the-art decentralized parallel stochastic gradient descent (D-PSGD)~\cite{jia2018highly,tang2018d,elgabli2019gadmm,xin2019decentralized,koloskova2019decentralized,lian2018asynchronous,hegedHus2019gossip,lalitha2019peer} using peer-to-peer communication in a connected graph still suffers from the low-speed links even though solves the communication bottleneck at the parameter server, as shown in \autoref{fig:example-bottleneck}(b).
%
%%%wyc: the synchronous and asynchronous might need explanation
D-PSGD can be further classified into synchronous and asynchronous.
%
In synchronous D-PSGD approaches, such as AllReduce-PSGD~\cite{jia2018highly} and D2~\cite{tang2018d}, the worker nodes communicate with their neighbors to exchange information at each iteration and they have to wait for the completion of all communications.
%
Thus, the whole training progress is constrained by the links with the lowest speed.
%
% Dumi: the below one needs a citation
This is known as the straggler problem\cite{luo2020prague}\cite{lian2018asynchronous}.
%
In asynchronous D-PSGD, such as GoSGD~\cite{hegedHus2019gossip}, AD-PSGD \cite{lian2018asynchronous} and Prague \cite{luo2020prague}, worker nodes perform the training independently. 
%
A worker node can randomly choose one or multiple neighbors to communicate with and start its next iteration once the communication is finished without waiting for others. 
%
However, as the neighbor selection follows an uniform probability distribution, a worker node may frequently select the neighbors with low-speed links, resulting in long communication time per iteration on average. 

To solve the above problems, namely the centralized communication bottleneck, straggler problem, and frequent communication via low-speed links, we design a novel Network-aware Asynchronous D-PSGD (\ourtech{}) approach with the following novel features.
%
(1) Worker nodes iteratively and asynchronously train model copies on their local data to avoid the straggler problem.
%
(2) Worker nodes exchange information via peer-to-peer communication to avoid centralized communication bottleneck.
%
(3) Each worker node randomly selects only one neighbor to exchange information per iteration and neighbors with high-speed links are selected with high probability.
%
This enables worker nodes to communicate preferably via high-speed links and, thus, reduce the communication time.

The design of such a decentralized learning approach faces the following three key challenges. 
%
\textbf{(1) Model consensus.} As decentralized training does not use a centralized node to synchronize the training of distributed worker nodes, the worker nodes may fall into different local optima, leading to great difference between worker nodes' model parameters and, as a consequence, failing to train a high-quality model. 
%
\textbf{(2) Fast convergence.} By simply assigning a high communication probability to neighbors with high-speed links, the worker node achieves low communication time 
but lacks the information from neighbors with low-speed links, leading to a low convergence rate. 
%
That is, much more communication rounds are needed to achieve convergence and this leads to increased convergence time. 
%
% Dumi: are you sure about the sentence below? It's not intuitive for me. Did you mean uniform selection?
On the other hand, simply assigning a high probability to neighbors with low-speed links can achieve good convergence rate. 
%
But the communication time per iteration is increased, leading to a long convergence time. 
%
Hence, there needs to be a trade-off between communication time and convergence rate to effectively reduce the convergence time. 
%
\textbf{(3) Network dynamic.} The link speeds between worker nodes may change during the training due to the dynamic arriving/leaving of other jobs and other communications in the network.
%
The initial communication probabilities may slow down the training since a high-speed link may become a low-speed link due to network competition with other jobs. 
%
Thus, the training should be adaptive to the network dynamic.  

% Dumi: do you theoretically prove "the models of all the worker nodes can reach consensus"?
% Zhou Pan: Yes. Thereom 1 and 2 are related to the consensus of models.
For the first challenge, we formulate the decentralized training as a consensus optimization problem and design a corresponding consensus stochastic gradient descent (SGD) algorithm. Each worker node performs the consensus SGD to iteratively update the local model using its local gradients and the difference between the local model and the one pulled from a selected neighbor. By doing so, the model differences between each pair of neighbors can be minimized and, finally, the models of all the worker nodes can reach consensus. We formally prove that our algorithm leads to consensus.
%
For the second challenge, we analyze the relationship between the convergence of the consensus SGD and the communication probabilities for selecting neighbors. Based on this analysis, we design an algorithm to generate a communication policy that seeks a trade-off between communication time and convergence rate to minimize the total convergence time. 
%
For the third challenge, we use the iteration time of worker nodes communicating with different neighbors to perceive the network condition and periodically update the communication policy to adapt to the dynamic network changes.

The main contributions of this paper are as follows.

\begin{itemize}

\item We identify the challenges of machine learning over a heterogeneous network and propose a Network-aware Asynchronous D-PSGD approach, namely \ourtech{}, to fully utilize fast links and speed up the training. 
\ourtech{} consists of novel (1) SGD consensus algorithm and (2) communication policy generation. 
The consensus algorithm guarantees that worker nodes synchronize their local model copies. 
The communication policy generation algorithm enables the worker nodes to communicate preferably via high-speed links and, thus, accelerate the training.

%\item The communication policy generation algorithm is designed such that it can also be applied to existing decentralized training frameworks, such as AD-PSGD~\cite{lian2018asynchronous} and GoSGD~\cite{hegedHus2019gossip}.

\item We theoretically prove that \ourtech{} provides convergence guarantees for decentralized training.

\item We implement \ourtech{} and evaluate it on a heterogeneous multi-tenant cluster. 
Experimental results show that \ourtech{} achieves speedups of 3.7$\times$, 3.4$\times$ and 1.9$\times$ comparing against state-of-the-art, namely Prague, Allreduce-SGD and AD-PSGD, respectively.
\end{itemize}

The rest of the paper is organized as follows. Section~\ref{sec:preliminaries} formulates our decentralized training problem. Section~\ref{sec:design} presents the design of \ourtech{}. Section~\ref{sec:convergence-analysis} provides the theoretical analysis of \ourtech{}. Section~\ref{sec:eval} evaluates \ourtech{} over both homogeneous and heterogeneous networks, Section~\ref{sec:relwork} presents related works and Section~\ref{sec:conclusion} concludes the paper.
